The MUSCLES Treasury Survey III: X-ray to Infrared Spectra of 11 M and K Stars Hosting Planets

We present a catalog of panchromatic spectral energy distributions (SEDs) for 7 M and 4 K dwarf stars that span X-ray to infrared wavelengths (5 {\AA} - 5.5 {\mu}m). These SEDs are composites of Chandra or XMM-Newton data from 5 - ~50 {\AA}, a plasma emission model from ~50 - 100 {\AA}, broadband empirical estimates from 100 - 1170 {\AA}, HST data from 1170 - 5700 {\AA}, including a reconstruction of stellar Ly{\alpha} emission at 1215.67 {\AA}, and a PHOENIX model spectrum from 5700 - 55000 {\AA}. Using these SEDs, we computed the photodissociation rates of several molecules prevalent in planetary atmospheres when exposed to each star's unattenuated flux ("unshielded" photodissociation rates) and found that rates differ among stars by over an order of magnitude for most molecules. In general, the same spectral regions drive unshielded photodissociations both for the minimally and maximally FUV active stars. However, for ozone visible flux drives dissociation for the M stars whereas NUV flux drives dissociation for the K stars. We also searched for an FUV continuum in the assembled SEDs and detected it in 5/11 stars, where it contributes around 10% of the flux in the range spanned by the continuum bands. An ultraviolet continuum shape is resolved for the star {\epsilon} Eri that shows an edge likely attributable to Si II recombination. The 11 SEDs presented in this paper, available online through the Mikulski Archive for Space Telescopes, will be valuable for vetting stellar upper-atmosphere emission models and simulating photochemistry in exoplanet atmospheres.

==> submission arxiv 2016-04-15/apecparams.tex <==
\tablehead{\ch{Star} & \ch{$kT$\tnm{a}} & \ch{$EM_{i}/EM_1$\tnm{b}} & \ch{$F_X$\tnm{c}}\\
 & \ch{[keV]} &  & \ch{[$10^{-14}$ erg s$^{-1}$ cm$^{-2}]$}}
		    
\startdata
GJ 1214 & 0.2\tnm{d} &  & $\leq 0.11$ \\
GJ 876 & $0.80 \pm 0.14$ &   & $9.1 \pm 0.8$ \\
 & $0.14 \pm 0.04$ & $3.5 \pm 4.6$ & \\
GJ 436 & $0.39 \pm 0.03$ &  & $1.2 \pm 0.1$ \\
GJ 581 & $0.26 \pm 0.02$ &  & $1.8 \pm 0.2$ \\
GJ 667C & $0.41 \pm 0.03$ &  & $3.9 \pm 0.3$ \\
GJ 176 & $0.31 \pm 0.02$ &  & $4.8 \pm 0.3$ \\
GJ 832 & $0.38_{-0.07}^{+0.11}$ &  & $6.2_{-0.7}^{+0.8}$ \\
 & $0.09_{-0.09}^{+0.02}$ & $4.8_{-2.9}^{+2.6}$ & \\
HD 85512 & $0.25_{-0.03}^{+0.04}$ &  & $1.9_{-0.3}^{+0.4}$ \\
HD 40307 & $0.15 \pm 0.06$ &  & $1.0\pm0.2$ \\
HD 97658\tablenotemark{e} & \nodata & \nodata & \nodata \\
\epseri & $0.70_{-0.07}^{+0.04}$ &  & $940\pm10$ \\
 & $0.32\pm0.01$ & $3.6_{-0.9}^{+0.7}$ & \\
 & $0.12_{-0.02}^{+0.09}$ & $2.4_{-1.0}^{+2.0}$ & \\
\enddata

\tablenotetext{a}{Plasma temperature. Multiple values for an entry represent multiple plasma components in the model.}
\tablenotetext{b}{For multi-component plasmas, this represents the ratio of the emission measure of the $i^\mathrm{th}$ component to the first component according to the order listed in the $kT$ column. }
\tablenotetext{c}{Flux integrated over full instrument bandpass.}
\tablenotetext{d}{Estimate is not well constrained and is based on an earlier \scraft{XMM-Newton} observation. See Section \ref{sec:exceptions}.}
\tablenotetext{e}{No observations. See Section \ref{sec:exceptions}.}

==> submission arxiv 2016-04-15/dissrates.tex <==
\tablehead{\colhead{Star} & \colhead{H$_2$} & \colhead{N$_2$} & \colhead{O$_2$} & \colhead{O$_3$} & \colhead{H$_2$O} & \colhead{CO} & \colhead{CO$_2$} & \colhead{CH$_4$} & \colhead{N$_2$O} & \colhead{O$_2$/O$_3$\tnm{a}}\\\colhead{} & \colhead{$\sn{-7}$} & \colhead{$\sn{-6}$} & \colhead{$\sn{-6}$} & \colhead{$\sn{-4}$} & \colhead{$\sn{-5}$} & \colhead{$\sn{-6}$} & \colhead{$\sn{-5}$} & \colhead{$\sn{-5}$} & \colhead{$\sn{-7}$} & \colhead{}}
\startdata
GJ 1214 & 0.36 & 3.3 & 0.86 & 1.2 & 3.2 & 2.6 & 0.7 & 4.2 & 0.82 & 0.0069\\
GJ 876 & 0.49 & 2.6 & 4.2 & 1.4 & 3.0 & 2.0 & 0.54 & 4.1 & 2.4 & 0.031\\
GJ 436 & 1.2 & 3.7 & 1.2 & 1.9 & 3.3 & 2.6 & 0.69 & 4.5 & 0.85 & 0.0065\\
GJ 581 & 0.18 & 1.4 & 0.59 & 1.5 & 1.6 & 1.1 & 0.3 & 2.2 & 0.34 & 0.0039\\
GJ 667C & 3.1 & 8.9 & 1.6 & 3.0 & 7.6 & 6.2 & 1.6 & 10 & 1.1 & 0.0052\\
GJ 176 & 2.1 & 5.1 & 3.4 & 2.6 & 4.2 & 3.4 & 0.89 & 5.6 & 2.2 & 0.013\\
GJ 832 & 2.2 & 6.5 & 2.1 & 3.7 & 5.7 & 4.6 & 1.2 & 7.8 & 1.6 & 0.0057\\
HD 85512 & 6.6 & 8.1 & 1.1 & 5.6 & 3.9 & 4.5 & 1.0 & 5.4 & 1.1 & 0.002\\
HD 40307 & 17 & 17 & 1.1 & 15 & 5.5 & 8.0 & 1.6 & 7.5 & 1.4 & 0.00075\\
HD 97658 & 17 & 15 & 1.8 & 34 & 4.9 & 7.2 & 1.4 & 6.6 & 3.6 & 0.00052\\
$\mathrm{\epsilon}$ Eri & 40 & 33 & 5.0 & 29 & 8.4 & 15 & 2.7 & 11 & 5.4 & 0.0017\\
Sun & 0.56 & 1.1 & 2.5 & 81 & 1.1 & 0.67 & 0.13 & 0.88 & 13 & 0.0003\\
\enddata

\tablenotetext{b}{Ratio of the \OIII\ to \OII\ dissociation rates.}


==> submission arxiv 2016-04-15/fuvcont.tex <==
\tablehead{
\colhead{Star} & \colhead{FUV Continuum} & \colhead{Detection} & \colhead{Fraction}\\
\colhead{} & \colhead{Flux} & \colhead{Significance} & \colhead{of Flux\tablenotemark{a}}\\
\colhead{} & \colhead{[erg s$^{{-1}}$ cm$^{{-2}}$ \AA$^{{-1}}$]} & \colhead{$\sigma$} & \colhead{}}
\startdata
GJ 1214 & $-1.2 \pm 1.1 \sn{-15}$ & \nodata & -0.753\\
GJ 876 & $6.7 \pm 1.2 \sn{-15}$ & 5.7 & 0.080\\
GJ 436 & $1.1 \pm 1.4 \sn{-15}$ & \nodata & 0.082\\
GJ 581 & $-8 \pm 13 \sn{-16}$ & \nodata & -0.201\\
GJ 667C & $1.1 \pm 1.1 \sn{-15}$ & \nodata & 0.088\\
GJ 176 & $4.1 \pm 1.2 \sn{-15}$ & 3.5 & 0.070\\
GJ 832 & $6.4 \pm 1.1 \sn{-15}$ & 6.1 & 0.122\\
HD 85512 & $6.4 \pm 5.4 \sn{-15}$ & \nodata & 0.114\\
HD 40307 & $8.2 \pm 4.8 \sn{-15}$ & \nodata & 0.147\\
HD 97658 & $1.13 \pm 0.18 \sn{-14}$ & 6.3 & 0.201\\
$\mathrm{\epsilon}$ Eri & $8.128 \pm 0.038 \sn{-13}$ & 215.9 & 0.128\\
\enddata



==> submission arxiv 2016-04-15/photrefs.tex <==
\tablehead{\colhead{Star} & \colhead{Photometry References}}
\startdata
GJ 1214 & 1,2,3,4,5,6,7,8,9\\
GJ 876 & 10,11,12,7,13,6,14,15,16,3,17,18,19,20,9\\
GJ 436 & 21,22,12,2,7,13,14,3,17,6,19,23,9\\
GJ 581 & 10,21,1,24,7,13,17,12,14,19,23,9\\
GJ 667C & 25,26,27\\
GJ 176 & 11,22,7,13,6,14,15,16,12,18,19,9\\
GJ 832 & 28,10,29,30,7,13,14,16,31,32,23,19,33,8,9\\
HD 85512 & 28,34,35,36,37,30,23,13,14,31,18,32,33,8,9\\
HD 40307 & 28,34,35,11,37,30,23,13,9,3,18,32,33,8,38\\
HD 97658 & 11,37,30,3,13,39,31,18,32,33,8,9\\
$\mathrm{\epsilon}$ Eri & 35,37,30,40,41,13,14,42,9,18,32,33,8,43\\
\enddata


\tablerefs{(1) \citealt{2004AAS...205.4815Z}; (2) \citealt{2014MNRAS.444..711T}; (3) \citealt{2013A&A...556A.150S}; (4) \citealt{2011PASP..123..412W}; (5) \citealt{2014yCat.2328....0C}; (6) \citealt{2012ApJ...748...93R}; (7) \citealt{2011AJ....142..138L}; (8) \citealt{2012yCat.2311....0C}; (9) \citealt{2003yCat.2246....0C}; (10) \citealt{2015AJ....149....5W}; (11) \citealt{2006ApJ...638.1004A}; (12) \citealt{2012A&A...546A..61D}; (13) \citealt{2008A&A...488..401R}; (14) \citealt{2003ApJ...582.1011S}; (15) \citealt{2004AJ....127.3043Z}; (16) \citealt{2013A&A...549A.109B}; (17) \citealt{2009ApJ...704..975J}; (18) \citealt{2010PASP..122.1437P}; (19) \citealt{2014MNRAS.443.2561G}; (20) \citealt{2014AJ....148..119F}; (21) \citealt{2010AJ....139.2440R}; (22) \citealt{2004AJ....128..463R}; (23) \citealt{2015A&C....10...99A}; (24) \citealt{2009ApJ...705.1226B}; (25) \citealt{2005yCat.2263....0T}; (26) \citealt{2013A&A...553A...8D}; (27) \citealt{2012yCat.1322....0Z}; (28) \citealt{2011AJ....142...15G}; (29) \citealt{2013A&A...551A..36N}; (30) \citealt{2007A&A...474..653V}; (31) \citealt{2015yCat.5145....0M}; (32) \citealt{2012AstL...38..331A}; (33) \citealt{2001KFNT...17..409K}; (34) \citealt{2009ApJ...705...89L}; (35) \citealt{2009A&A...501..941H}; (36) \citealt{2012ApJS..200...15A}; (37) \citealt{2010A&A...515A.111S}; (38) \citealt{2013A&A...555A..11E}; (39) \citealt{2011MNRAS.411..435B}; (40) \citealt{2002A&A...384..180F}; (41) \citealt{2009ApJS..184..138H}; (42) \citealt{2010AJ....139.1242A}; (43) \citealt{1879RNAO....1.....G}}


==> submission arxiv 2016-04-15/starprops.tex <==
\tablehead{ \colhead{Star} & \colhead{Type} & \colhead{$d$} & \colhead{V} & \colhead{ref} & \colhead{MUSCLES $T_{eff}$} & \colhead{Literature $T_{eff}$} & \colhead{ref} & \colhead{$\log{g}$} & \colhead{ref} & \colhead{$\left [ Fe/H \right ] $} & \colhead{ref} \\ \colhead{} & \colhead{} & \colhead{[pc]} & \colhead{} & \colhead{} & \colhead{[K]} & \colhead{[K]} & \colhead{} & \colhead{[[cm s$^{-2}$]} & \colhead{} & \colhead{} & \colhead{} }
\startdata
GJ 1214 & M4.5 & 14.6 & $ 14.68 \pm 0.02 $ & 1 & $ 2935 \pm 100 $ & $ 2817 \pm 110 $ & 2 & $ 5.06 \pm 0.52 $ & 3 & $ 0.05 \pm 0.09 $ & 2\\
GJ 876 & M5 & 4.7 & $ 10.192 \pm 0.002 $ & 4 & $3062_{-130}^{+120}$ & $ 3129 \pm 19 $ & 5 & $ 4.93 \pm 0.22 $ & 3 & $ 0.14 \pm 0.09 $ & 2\\
GJ 436 & M3.5 & 10.1 & $ 10.59 \pm 0.08 $ & 6 & $ 3281 \pm 110 $ & $3416_{-61}^{+54}$ & 7 & $ 4.84 \pm 0.16 $ & 3 & $ -0.03 \pm 0.09 $ & 2\\
GJ 581 & M5 & 6.2 & $ 10.61 \pm 0.08 $ & 6 & $ 3295 \pm 140 $ & $ 3442 \pm 54 $ & 8 & $ 4.96 \pm 0.25 $ & 3 & $ -0.20 \pm 0.09 $ & 2\\
GJ 667C & M1.5 & 6.8 & 10.2 & 9 & $ 3327 \pm 120 $ & $ 3445 \pm 110 $ & 2 & $ 4.96 \pm 0.25 $ & 3 & $ -0.50 \pm 0.09 $ & 2\\
GJ 176 & M2.5 & 9.3 & 10.0 & 10 & $ 3416 \pm 100 $ & $ 3679 \pm 77 $ & 5 & $ 4.79 \pm 0.13 $ & 3 & $ -0.01 \pm 0.09 $ & 2\\
GJ 832 & M1.5 & 5.0 & 8.7 & 10 & $ 3816 \pm 250 $ & $ 3416 \pm 50 $ & 11 & $ 4.83 \pm 0.15 $ & 3 & $ -0.17 \pm 0.09 $ & 2\\
HD 85512 & K6 & 11.2 & 7.7 & 10 & $4305_{-110}^{+120}$ & $ 4400 \pm 45 $ & 12 & $ 4.4 \pm 0.1 $ & 12 & $ -0.26 \pm 0.14 $ & 12\\
HD 40307 & K2.5 & 13.0 & 7.1 & 10 & $ 4783 \pm 110 $ & $ 4783 \pm 77 $ & 12 & $ 4.42 \pm 0.16 $ & 12 & $ -0.36 \pm 0.02 $ & 12\\
HD 97658 & K1 & 21.1 & 7.7 & 10 & $ 5156 \pm 100 $ & $ 5170 \pm 50 $ & 13 & $ 4.65 \pm 0.06 $ & 14 & $ -0.26 \pm 0.03 $ & 14\\
$\mathrm{\epsilon}$ Eri & K2.0 & 3.2 & 3.7 & 15 & $ 5162 \pm 100 $ & $ 5049 \pm 48 $ & 12 & $ 4.45 \pm 0.09 $ & 12 & $ -0.15 \pm 0.03 $ & 12\\
\enddata


\tablerefs{(1) \citealt{weis96}; (2) \citealt{neves14}; (3) \citealt{santos13}; (4) \citealt{landolt09}; (5) \citealt{braun14}; (6) \citealt{hog00}; (7) \citealt{braun12}; (8) \citealt{boyajian12}; (9) \citealt{mermilliod86}; (10) \citealt{koen10}; (11) \citealt{houdebine10}; (12) \citealt{tsantaki13}; (13) \citealt{grootel14}; (14) \citealt{valenti05}; (15) \citealt{ducati02}}


==> submission arxiv 2016-04-15/x-ray_alex.tex <==
\subsection{X-ray data}


We obtained X-ray data with \scraft{XMM-Newton} for GJ 832, HD 85512, HD 40307, and \epseri\ and with \scraft{Chandra} for GJ 1214, GJ 876, GJ 581, GJ 436, and GJ 176. 
Complete details of the X-ray data reduction and an analysis of the results will be presented in a follow-on paper (\citealt{brown16}; in prep.). 
Here we provide a brief outline of the reduction process. 
The technique used to observe X-ray photons imposes some challenges to  extracting the source spectrum from the observational data.
The X-ray emission was observed using CCD detectors that have much lower spectral resolution ($\lambda / \Delta \lambda \sim$ 10-15 for the typical 1 keV photons observed from the MUSCLES stars) than the spectrographs used to measure the UV and visible spectra. 
The data were recorded in instrumental modes designed to allow the efficient rejection of particle and background photon events. 
CCD X-ray detectors have very complex instrumental characteristics that are energy-dependent and also depend critically on where on the detector a source is observed.
Broad, asymmetric photon energy contribution functions result from these effects, and it is nontrivial to associate a measured event energy to the incident photon energy. 
Consequently, simply assigning to each detection the most likely energy of the photon that created the detected event and binning in energy does not accurately reproduce the source spectrum.


To estimate the true source spectrum, we used the XSPEC software package \citep{arnaud96} to forward model and  parameterize the observed event list, using model spectra generated by APEC (Astrophysical Plasma Emission Code; \citealt{smith01}). 
For each spectrum, we experimented with fits to plasma models containing one to three temperature components and with elemental abundance mixes that were either fixed to solar values or free to vary (but normally only varying the Fe abundance, because it is the dominant emission line contributor) until we achieved the most reasonable statistical fit. The complexity of the model fit is strongly controlled by the number of detected X-ray events. The resulting model parameters are listed in Table \ref{tbl:xfitparams}.


We then computed the ratio of the number of photons incident in each energy bin to the number actually recorded, and corrected the measured photon counts accordingly. 
The spectral bin widths are variable because the data were binned to contain an equal number of counts per energy bin.


%UPDATE!!!
\begin{deluxetable}{lccc}
\tablewidth{0pt}
\tablecaption{Parameters of the APEC model fits to the X-ray data. \label{tbl:xfitparams}}

\input{apecparams.tex}

\end{deluxetable}


The X-ray data do not extend to the start of the EUV region, and this 
results in an energy distribution  
gap that, depending on the S/N of the X-ray observations, starts 
at 30~--~60~\AA\ and ends where the empirical EUV flux estimates \mychng{(see Section \ref{sec:lyareduction})} 
begin at 100~\AA. We filled this gap with the output of the same best-fit 
APEC model that yielded the count-rate corrections for the measured 
X-ray spectrum.

